ELEVATER: A Benchmark and Toolkit for Evaluating Language-Augmented Visual Models

Learning visual representations from natural language supervision has recently shown great promise in a number of pioneering works. In general, these language-augmented visual models demonstrate strong transferability to a variety of datasets and tasks. However, it remains challenging to evaluate the transferablity of these models due to the lack of easy-to-use evaluation toolkits and public benchmarks. To tackle this, we build ELEVATER (Evaluation of Language-augmented Visual Task-level Transfer), the first benchmark and toolkit for evaluating(pre-trained) language-augmented visual models. ELEVATER is composed of three components. (i) Datasets. As downstream evaluation suites, it consists of 20 image classification datasets and 35 object detection datasets, each of which is augmented with external knowledge. (ii) Toolkit. An automatic hyper-parameter tuning toolkit is developed to facilitate model evaluation on downstream tasks. (iii) Metrics. A variety of evaluation metrics are used to measure sample-efficiency (zero-shot and few-shot) and parameter-efficiency (linear probing and full model fine-tuning). ELEVATER is a platform for Computer Vision in the Wild (CVinW), and is publicly released at at https://computer-vision-in-the-wild.github.io/ELEVATER/

==> subtex/checklist.tex <==
\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} See Appendix Section~\ref{sec:societal}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
   \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
   \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}, in Appendix Section~\ref{sec:appendix_benchmark}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}, in Appendix Section~\ref{sec:appendix_benchmark}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}, in Appendix Section~\ref{sec:appendix_benchmark}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> subtex/main_arxiv.tex <==
\maketitle

\begin{abstract}

Learning visual representations from natural language supervision has recently shown great promise in a number of pioneering works. In general, these language-augmented visual models demonstrate strong transferability to a variety of datasets/tasks.
However, it remains a challenge to evaluate the transferablity of these foundation models due to the lack of easy-to-use toolkits for fair benchmarking. To tackle this, we build \shortname{}\blfootnote{$^*$Equal Technical Contribution\hspace{3mm}$^\spadesuit$Project Lead}\footnote{\longname{}}, the first benchmark to compare and evaluate pre-trained language-augmented visual models. Several highlights include:
$(i)$ Datasets. As downstream evaluation suites, it consists of 20 image classification datasets and 35 object detection datasets, each of which is augmented with external knowledge.
$(ii)$ Toolkit. An automatic hyper-parameter tuning toolkit is developed to ensure the fairness in model adaption. To leverage the full power of language-augmented visual models, novel language-aware initialization methods are proposed to significantly improve the adaption performance.
$(iii)$ Metrics. A variety of evaluation metrics are used, including sample-efficiency (zero-shot and few-shot) and parameter-efficiency (linear probing and full model fine-tuning).
We will release our toolkit and evaluation platforms for the research community.
\end{abstract}


\section{Introduction}
Visual recognition has become ubiquitous in our society~\cite{szeliski2010computer}, with applications in geo-localization~\cite{radford2021learning}, action recognition~\cite{soomro2012ucf101}, street number transcription~\cite{netzer2011reading}, satellite remote sensing~\cite{helber2019eurosat}, medical imaging~\cite{Veeling2018-qh},  self-driving cars~\cite{geiger2013vision}, etc. Core to many of these applications are visual recognition tasks such as image classification (IC) and object detection (OD). It is of high value to develop transferable visual models that perform well on a wide range of downstream application scenarios.
By leveraging large web crawled image-text corpora, recent advances in language-augmented visual models such as  CLIP~\cite{radford2021learning} and ALIGN~\cite{jia2021scaling} have demonstrated strong transfer performance, making this direction arguably the most practical visual learning approach, because
$(i)$ open-set recognition is enabled due to the problem reformulation from classification to retrieval; $(ii)$ generalization is improved since the form of language supervision allows higher coverage of visual concepts.

The success has quickly inspired many follow-up large-scale pre-training works~\citep{yang2022unicl,yuan2021florence,yao2021filip,li2021supervision,mu2021slip,gu2021zero,li2021grounded,zhong2021regionclip}. Each of them developed their own evaluation experiments, covering a customized subset of tasks, and leaving the details of model adaptation process less accessible. These tasks are often studied repeatedly in isolation, and require a lot of development effort to work. 
%
To fill this gap, in this paper we develop an open-resource benchmark and toolkit, designed to make working on task-level transfer easier, more vigorous, and reproducible. We provide software to evaluate models without task-specific tuning, and also comprehensive metrics to measure model performance from various perspectives.

Our main findings and contributions can be summarized as follows:

\begin{itemize}[leftmargin=5.5mm]

\item {\bf Benchmark: Datasets and Knowledge.} 
We build the first publicly available benchmark to evaluate the recent language-augmented visual models. It includes a suite of 20 and 35 datasets for image classification (IC) and object detection (OD), respectively.
Beyond that, external knowledge is collected for each dataset to further augment language, including WordNet hierarchy~\citep{miller1998wordnet}, WordNet definition~\citep{miller1998wordnet}, Wiktionary definition~\cite{meyer2012wiktionary}, and GPT-3 knowledge~\cite{brown2020language}, which represents the first comprehensive benchmark in evaluating {\em large-scale task-level transfer}. 

\item {\bf Comprehensive Metrics.} To take into account the practical efficiency in the deployment stage in the real world, a variety of evaluation metrics are developed with the full sample and parameter spectrum in mind. Specifically, we include sample-efficiency (zero-shot, few-shot and full-shot) and parameter-efficiency (linear probing and full model fine-tuning) in experiments.

\item {\bf Reproducible Toolkit \& Language-augmented Adaptation Methods.} 
We develop an open-source software toolkit to support model adaptation and evaluation. Automatic hyper-parameter tuning is employed to avoid human-in-the-loop tuning, thus reducing human labor and ensuring fair comparisons of different model checkpoints. 
We propose new model adaptation methods to leverage the full power of pre-trained language-augmented visual models, which significantly outperform the traditional vision-only adaptation method in all settings. All these methods are implemented as strong baselines, serving as a starting tutorial to encourage more advanced adaptation solutions.

\item {\bf Novel Empirical Findings.} Several of our observations challenge previously reported results. 
$(i)$ Random initialization of the linear head in language-augmented visual models is sub-optimal; instead, leveraging both text and vision in these models consistently yields better performance. Importantly, few-shot always performs better than zero-shot, in contrast to the results reported in~\cite{radford2021learning}.
$(ii)$ For language-augmented visual models, linear probing consistently performs better than full model fine-tuning in the data-limited settings. As the training dataset size increases, fine-tuning gradually overtakes linear probing. In contrast, for traditional language-free models, fine-tuning always performs better.
$(iii)$ External knowledge can benefit zero-shot and few-shot learning performance, when used properly. Further, the implicit knowledge generated by GPT3~\cite{brown2020language} improves the zero-shot performance.
\end{itemize}



\section{Related Work}

\subsection{Visual Recognition Benchmarks: Zero-shot and Transfer Learning} 
Zero-shot learning in computer vision has been studied for decades. The research topic has witnessed two types of distinctive notions of zero-shot: the traditional {\it class-level zero-shot} that usually refers to the study of generalizing to unseen object categories~\cite{lampert2009learning}, and the recently popular {\it task-level zero-shot} that refers to the study of generalizing to unseen datasets/tasks~\cite{li2017learning,radford2021learning}.
In Table~\ref{tab:dataset}, we compare our benchmark against existing benchmarks.
Existing zero-shot learning benchmarks are developed for the class-level zero-shot setting. They are usually in single domain, with a manual split of categories to product disjoint training and test categories, \eg Animal with Attributes (AwA)~\citep{lampert2013attribute}, Caltech-UCSD Birds-200 (CUB)~\cite{wah2011caltech}, SUN~\cite{patterson2012sun}, aPY~\cite{farhadi2009describing}, and ZS-ImageNet~\cite{rohrbach2011evaluating,fu2016semi}. 
%ensure certain disjoint between training and test categories

In contrast, our benchmark focuses on task-level transfer across domains, \ie it aims to evaluate the transferability of models, by pre-training from their own large corpus, then evaluating zero-shot performance on a diverse set of downstream datasets. This setting has been recently studied~\cite{li2017learning,radford2021learning,li2021align,yuan2021florence}, and is arguably more practical for real-world applications, as it brings the convenience towards the spirit of one-model-for-all. 
The well-known ImageNet-1K dataset~\cite{deng2009imagenet} was originally proposed as a large dataset for model training and testing. It has also recently been considered as one downstream task to study zero-shot transfer~\cite{radford2021learning,li2021align,yuan2021florence}.
Our work presents the first \emph{public benchmark} to standardize the zero-shot task-level transfer setting. Note that visual task transfer has been previously explored in VTAB~\cite{zhai2019large}, which measures good visual representations as those that adapt to diverse, unseen tasks with an emphasis on few examples. The pre-trained models and task adaptation in VTAB are considered for vision backbones only, and no language model/modality is involved.
Our benchmark shares a similar spirit of task-level transfer to VTAB, but strives for analyzing the vital importance of language and knowledge in visual transfer.
%
We have further made several novel contributions to consolidate the benchmark: $(i)$ We add external knowledge for each dataset to cultivate new research directions in knowledge-augmented visual models, inspired by the success of knowledge in traditional class-level transfer. $(ii)$ We consider the full spectrum in measuring the sample-efficiency of task adaptation, including zero-shot, few-shot, and full-shot.



% It belongs to generalized zero-shot settings, but more practical as it emphasizes transfer learning on a wide range of datasets: a model that performs well on 20 diverse tasks.

% , , , ,

\begin{table}[t]
    \centering
    \footnotesize
\setlength{\tabcolsep}{2.5pt}
 \scalebox{0.91}{
    \begin{tabular}{l | l cccc | c c c }
    \toprule
    &  \multicolumn{5}{c}{\bf Benchmark Statistics}   &  \multicolumn{2}{|c}{\bf Evaluation Settings}  \\
   Problem &  & \#Datasets &  \#Image & \#Concepts & Knowledge Source &  Zero & Few & Full  \\
    \midrule
     \multirow{5}{*}{IC}
    & AwA~\citep{lampert2013attribute} & 1 & 30337 / 6985   & 40 / 10  & Attributes  & $\checkmark$ &   &   \\
    & CUB~\cite{wah2011caltech} & 1 &  8855 / 2933  & 150 / 50  & Attributes  & $\checkmark$ &   &  \\
    & SUN~\cite{patterson2012sun}  & 1 &  12900 / 1440  & 645 / 72  & Attributes  & $\checkmark$ &   &  \\
    & aPY~\cite{farhadi2009describing}  & 1 &  12695 / 2644  &  20 / 12  & Attributes  & $\checkmark$ &   &  \\
    & ZS-ImageNet~\cite{rohrbach2011evaluating}  & 1 &  1.2M / 54K  &  1K / 360 &  WordNet & $\checkmark$ &   &  \\
    & ImageNet-1K~\cite{deng2009imagenet}  & 1 &  1.2M / 50K  &  1K &  WordNet & $\checkmark$ &   & $\checkmark$ \\   
    & VTAB~\cite{zhai2019large}  & 19 &  2.2M / -  &  940 &  - &  & $\checkmark$  & $\checkmark$ \\       
    & \cellcolor{Gray}\shortname{} (Ours) &
    \cellcolor{Gray}20 &
    \cellcolor{Gray}638K / 193K &
    \cellcolor{Gray}1151$^{\diamondsuit}$ &
    \cellcolor{Gray}WordNet, Wiki, GPT-3  &
    \cellcolor{Gray}$\checkmark$ &
    \cellcolor{Gray}$\checkmark$ &
    \cellcolor{Gray}$\checkmark$ \\    
    \midrule
    \multirow{2}{*}{OD}
    & LVIS~\cite{gupta2019lvis} &  1 &  120k / 40K  & 1723  & WordNet &  &   &  $\checkmark$ \\
    & \cellcolor{Gray}\shortname{} (Ours) &  
    \cellcolor{Gray}35 &  
    \cellcolor{Gray}132K / 20K &  
    \cellcolor{Gray}314$^{\diamondsuit}$  & 
    \cellcolor{Gray}WordNet, Wiki, GPT-3 & \cellcolor{Gray}$\checkmark$ &
    \cellcolor{Gray}$\checkmark$ &
    \cellcolor{Gray}$\checkmark$ \\   
    \bottomrule
    \end{tabular}
    }
    \vspace{2pt}
    \caption{Comparison of dataset statistics and evaluation settings. For existing zero-shot datasets in IC, the numbers of images and concepts are reported for development and evaluation stages separately. $^{\diamondsuit}$ It represents the total \#concepts in the benchmark to evaluate task-level transfer, and there is no train-evaluation category split as in class-level transfer.}
    \label{tab:dataset}
    \vspace{-0mm}
\end{table}

% \subsection{Language-Image Training Methods.} 

\subsection{Pre-trained Models in NLP: Benchmarks, Adaptation, and Knowledge} 
Our work takes major inspiration from the development of pre-trained language models in natural language processing (NLP) in several aspects:
$(i)$
{\it Benchmarks}. Platforms with a suite of small datasets such as GLUE~\cite{wang2018glue}/SuperGLUE~\cite{wang2019superglue} have been extensively used to evaluate the general language understanding ability of pre-trained models~\cite{devlin2018bert}. Recently, there is a trend in NLP to develop task-agnostic models such as the GPT family~\cite{brown2020language} that demonstrate task-level transfer learning ability, enabling zero-shot and few-shot transfer to downstream datasets. The success in NLP encourages us to build a generic benchmark to measure the similar transferability for visual models.
$(ii)$
{\it Efficient adaptation}. The democratization of large pre-trained models for efficient adaptation in downstream applications is an important topic in practice. Many algorithms have been developed for various efficiency considerations, including adapters~\cite{houlsby2019parameter} and prompt tuning~\cite{li2021prefix,liu2021pre}. It has inspired a few recent works for language-augmented visual models~\citep{zhou2022conditional,sung2021vl,yao2021cpt,gao2021clip}. Our benchmark can serve as a comprehensive playground to quantify the progress in the emerging field of visual model adaptation. We also propose a novel language-initialized adaptation method as a strong baseline. 
$(iii)$
{\it Knowledge}. Knowledge-intensive tasks~\cite{marino2019ok,petroni2020kilt} — those where a human can only be expected to perform the task with access to a knowledge source such as Wikipedia — are challenging for even cutting edge NLP and vision-and-language models, as it is infeasible to train large models to memorize everything. KILT~\cite{petroni2020kilt} is a benchmark that contains a suite of tasks/datasets for evaluating and analyzing knowledge-intensive NLP models. Similarly, we also add various external knowledge sources in each downstream dataset for our vision benchmark.

\section{Benchmarks}

\subsection{A Suite of Datasets with Language/Knowledge Augmentations}

As a proxy for performing unseen tasks in the wild, we collect a diverse set of public datasets from various domains in computer vision, as the basis of our benchmark. Specifically, we consider 20 datasets for IC and 35 datasets for OD. We exhibit the dataset names in Figure~\ref{fig:benchmark} (a), and the detailed statistics of each dataset in the Appendix. It is recommended in~\cite{radford2021learning} that studying task-level zero-shot transfer is a way of measuring the task learning capabilities of machine learning systems. The task definition of each downstream recognition dataset is typically specified using category names. Adding customer specification/note is a natural way to clarify the task definition \eg the attribute or explanation of a visual concept.
Importantly, a similar spirit has been implemented in traditional class-level zero-shot by adding individual domain-specific knowledge (see Table~\ref{tab:dataset}), and demonstrated promising zero-shot performance gains. In this paper, we generalize the terms to task-level, collecting external knowledge from general sources for our benchmark.

% as aspired to in the zero-data learning paper of

\begin{itemize}[leftmargin=2.5mm]
\vspace{-1mm}
\item \textit{WordNet Hierarchy}  ($\texttt{def\_path}$). The words along the traversal path from the query node in WordNet~\citep{miller1998wordnet} to the highest parent node is recorded as the hierarchy knowledge.
\vspace{-1mm}
\item \textit{WordNet Definition} ($\texttt{def\_wn}$). The definition in WordNet synsets~\citep{miller1998wordnet} is used to explain the query.
\vspace{-1mm}
%
\item \textit{Wiktionary Definition} ($\texttt{def\_wik}$). The definition of a query in  Wiktionary~\cite{meyer2012wiktionary} is used.
\vspace{-1mm}
\item \textit{GPT3 Knowledge} ($\texttt{gpt3}$). For the above three knowledge sources, it is not always feasible to retrieve valid knowledge for any query.  To enable full knowledge coverage, we propose to use GPT3~\cite{brown2020language} to generate ``pseudo'' knowledge, where the in-context-learning prompt is constructed with multiple pairs of class names and their Wiktionary definitions. We generate five GPT3 knowledge sequences for each class name, by constructing different context prompts with randomly sampled pairs.

\end{itemize}

\begin{figure}[t!]
    \centering
    \begin{subtable}[h]{1.0\textwidth} \centering
    \scalebox{1.0}{
    \begin{tabular}{cc}
    \hspace{-3mm}
     \includegraphics[width=.48\linewidth]{figs/benchmark_examples/word_cloud_ic.pdf}
     & 
     \hspace{-2mm}
     \includegraphics[width=.5\linewidth]{figs/benchmark_examples/word_cloud_od.pdf}
  \\
    \end{tabular}
    }
    \vspace{-2mm}
   \caption{Dataset names. The font size is proportional to the number of concepts in each dataset.}%indicates
	\label{fig:benchmark_dataset_names}
    \end{subtable}    
    %
    
    \begin{subtable}[h]{0.98\textwidth} \centering
    \vspace{2mm}
    \scalebox{1.0}{
    \begin{tabular}{cc}
    \hspace{-4mm}
     \includegraphics[width=.48\linewidth]{figs/benchmark_examples/benchmark_example_ic.pdf}
     & 
     \hspace{-4mm}
     \includegraphics[width=.51\linewidth]{figs/benchmark_examples/benchmark_example_od.pdf}
  \\
    \end{tabular}
    }
    \vspace{-2mm}
   \caption{Examples of collected external knowledge.}
	\label{fig:benchmark_examples}
    \end{subtable}    
    %
    \vspace{-0mm}
    \caption{Illustration of our benchmark. Left: Image classification, Right: Object detection.}
    \label{fig:benchmark}  
    \vspace{-4mm}
\end{figure}


In Fig.~\ref{fig:benchmark}~(b), we show examples to illustrate the knowledge sources. In practice, there is a trade-off between the knowledge quality and its coverage. For example, WordNet has relatively rich and precise knowledge, but the coverage is low; GPT3 knowledge has the full coverage (as it is generated via prompting a pre-trained neural language model), but it is hard to assess its quality. In the experiment section, we provide baseline results to demonstrate the benefits of external knowledge, and encourage the community to design advanced modeling/prompting techniques to leverage these knowledge sources.


\subsection{Pre-trained Models for Transfer Learning}

\paragraph{Industry Track and Academic Track.} Our benchmark is essentially an evaluation platform for pre-trained models, whose performance largely depends on the scale of the pre-training corpus. Larger corpus typically yields higher performance, but unfortunately results in a barrier to many participants, especially a majority of researchers from university labs. To increase inclusivity, we create two tracks with restrictions on the pre-training data scale: 
%prevent more
%
$(i)$
{\it Industry track} has no limit on pre-training data scale, except that images in our benchmark are not allowed in pre-training when reporting zero-/few-shot performance. This track aims to explore the scaling limit.
%
$(ii)$
{\it Academic track} is a setting that limits the data in established public large datasets (\ie ImageNet-21K~\cite{deng2009imagenet}, GCC3M~\cite{sharma2018conceptual} \& 12M~\cite{changpinyo2021conceptual}, YFCC15M~\cite{thomee2016yfcc100m}). This track is more academic-friendly, aiming to encourage the exploration in data-efficient pre-training methodologies. We encourage participants in this track to report the pre-training datasets to enable reproducible research.
%encourage
%
\paragraph{Image Classification}
We consider four checkpoints to produce baseline results for IC. The first two are for the industry track, the last two are for the academic track.

\begin{itemize}[leftmargin=2.5mm]
\item \textit{Supervised ViT-B32 }~\cite{dosovitskiy2020image} represents a checkpoint for the traditional language-free visual models, where model training is performed on ImageNet-22K with cross-entropy loss.
\vspace{-1mm}
%
\item \textit{CLIP ViT-B32}~\cite{radford2021learning} represents a checkpoint for the family of the language-augmented visual models, trained with 400M image-text pairs.
\vspace{-1mm}
%
\item \textit{UniCL Swin}~\cite{yang2022unicl} represents knowledge-free language-augmented visual models with Swin~\cite{liu2021Swin} as the visual backbone, trained in the academic setting with ImageNet-21K, which excludes ImageNet-1K categories from ImageNet-22K.
\vspace{-1mm}
%
\item \textit{Knowledge UniCL Swin}~\cite{shen2022klite} represents knowledge-enriched language-augmented visual models. Its pre-training setting is the same as UniCL Swin, but external knowledge such as Wiktionary is leveraged in model pre-training.
\end{itemize}

\paragraph{Object Detection}
We consider four checkpoints to produce baseline results for OD. They are for the academic track, as they are pre-trained on public datasets. All of them employ Swin-Tiny backbone~\cite{liu2021Swin}.
%
\begin{itemize}[leftmargin=2.5mm]
\item \textit{DyHead}~\cite{dai2021dynamic} represents a checkpoint for the traditional language-free object detector, where model  is pre-trained on Object365~\cite{shao2019objects365} without leveraging the category name information.
\vspace{-1mm}
%
\item \textit{GLIP}~\cite{li2021grounded} represents a checkpoint for the family of the language-augmented object detector, trained with Object365 and Flicker phrase grounding data~\cite{plummer2015flickr30k}.
\vspace{-1mm}
%
\item \textit{GLIP-A}~\cite{li2021grounded} represents knowledge-free language-augmented object detector, where model is trained on Object365 and the semantics of category names is leveraged.
\vspace{-1mm}
%
\item \textit{Knowledge GLIP-A}~\cite{shen2022klite} represents knowledge-enriched language-augmented object detector. Its training setting is the same as GLIP-A, except that Wiktionary knowledge is leveraged in model pre-training.
\end{itemize}

In summary, among four checkpoints for each problem, the first two are used to compare the state-of-the-art in language-free and language-augmented models, and latter two are used to compare the knowledge-free and knowledge-augmented models (both belongs to language-augmented models, as knowledge is presented as a structured form of language).

\subsection{Evaluation Settings: Efficiency Considerations}

\paragraph{Sample-efficiency: Zero-shot, Few-shot, and Full-shot.} Due to the high cost of annotating data, it is often desired to provide a small number of labeled image-label pairs for model adaptation in a downstream transfer dataset. Good models should be able to reach high performance in this data-limited scenario. To assess this ability, we construct a variety of settings, by varying the number of training set size $N$ in the downstream dataset.
For IC, $N=0, 5, 20, 50, |\Dcal|$, where $|\Dcal|$ is the total number of samples for a given dataset. For OD, $N=0, 1, 3, 5, 10, |\Dcal|$. Three random seeds are chosen, each of which identifies a subset of samples from the full dataset in a deterministic manner. In other words, once the random seed is given, the indices of training samples in few-shot settings are fixed to encourage reproducible research.

\paragraph{Parameter-efficiency: Linear Probing vs Full Model Fine-tuning.} Maintaining a small number of dataset-specific model parameters is often favored for model maintenance, as it can be expensive to maintain a unique copy of large model checkpoints for each of the thousands of downstream AI applications. In IC, linear probing provides a simple strategy for training a dataset-specific linear embedding matrix, while keeping the pre-trained visual backbone frozen. It arguably represents the minimum cost solution for parameter-efficient model adaptation. In contrast, fine-tuning often updates the entire weights in backbone and linear head, representing the most expensive solution to model adaptation. We implement these two representative solutions as baselines. In OD~\cite{wang2020frustratingly}, linear probing typically means updating the linear heads for classification and localization (including centers) tasks only, while fine-tuning means update all model weights including the backbone and the detectors.

\section{Toolkits}

\subsection{Automatic Hyper-parameter Tuning}
\paragraph{Image Classification.}
For a given dataset, we split its training set into training and validation with a ratio 80\% vs 20\%. At least one training sample per class is ensured for training and validation.  Grid search is applied over learning rate $\eta$  and weight decay $\alpha$. In the hyper-parameter search stage, the model is trained with a given configuration $(\eta, \alpha)$ for 10 epochs, the best hyper-parameter configuration is chosen as the one with the best validation performance along the entire process. After that, a final run is performed for 50 epochs to report the performance on the testing set.

\paragraph{Object Detection.} A validation set is chosen in the hyper-parameter search stage. We consider validation set size $(1, 1, 1, 3, full)$ for $N=1, 3, 5, 10, |\Dcal|$, respectively. For each type of checkpoints (DyHead, GLIP) and each adaption method, we have a set of pre-selected hyparameters, \ie batch size |$\mathcal{B}$|, initial learning rate $\eta_0$ and weight decay $\alpha$, as shown in Table~\ref{tab:odinw_hyperparams} in Appendix. They are determined by either empirical rules or simple hyper-parameter tuning. For each setting and each train/val split, we evaluate on the val split after every training epoch to decrease the learning rate in a step-wise manner. More specifically, we use the PyTorch {\it ReduceLROnPlateau} with patience 3 and factor 0.1 to decrease the learning rate when there is no improvement on val. We terminate the fine-tuning process if we do not see improvements for continuously 9 epochs, return the checkpoint with the best score on val, and report its score on the test split. For each few-shot setting, we random sample the train/val split 3 times, and report the average score and standard deviation on the test split. 




\subsection{Model Adaptation Methods}

\label{sec:model_adaptation}

We provide several model adaptation methods as strong baselines, which allow effective transfer learning of pre-trained visual models. The ideas are illustrated in Figure~\ref{fig:adaptation}. For a downstream dataset, we first represent it in a triplet-wise data format $\Dcal  = \{ (\xv_n, \tv_n, y_n) \}_{n=1}^N$, where $\xv \in \Xcal$  is the image, $\tv \in \Tcal$ is its corresponding language description, and $y \in \Ycal$ is a label indicating the index of the grouped or unique language description in the dataset. In IC, the number of labels $|\Ycal| = K$, the number of category names.  

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.99\linewidth]{figs/method_comparison.pdf}
% 	\includegraphics[width=0.99\linewidth]{figures/FocalNet-Fig1.pdf}	
    \vspace{-0mm}
    \caption{Illustrative comparison among different model evaluation and adaption methods.
    }
    \vspace{-0mm}
    \label{fig:adaptation}
\end{figure}


\paragraph{Language-free Visual Models.} Most existing visual models are language-free, as language information is often not considered in training, \eg supervised and self-supervised learning methods. Such models can not be directly used for zero-shot transfer, and model adaptation is often enabled by adding additional weights. For each image $\xv$, an image encoder model $f_{\thetav}$ parameterized by $\thetav$ first represents $\xv$ as a visual feature vector $ \hv \in \R^{D\times 1}$: $  \hv  = f_{\thetav}(\xv)$. A linear classifier with parameters $\Wmat \in \R^{D\times K}$ (we absorb the bias $\bv$ in $\Wmat$ for simplicity) is used, where $\Wmat$ is randomly initialized, shown in Figure~\ref{fig:adaptation} (a). 

\paragraph{Language-augmented Visual Models.} Recent works~\cite{radford2021learning,jia2021scaling} that learn visual models with language supervision often employ a two-encoder architecture. Besides the image encoder model $f_{\thetav}$, a text encoder $f_{\phiv}(\tv)$ parameterized by $\phiv$ is also used to encode text $\tv$. Additional projection layers $\Wmat_u$ and $\Wmat_v$ are introduced for image and language features, embedding them into a joint space with dimension $P$, with projected features as $\uv$ and $\vv$ respectively. As shown in Figure~\ref{fig:adaptation} (b), zero-shot learning can be directly performed in this space: the mean text feature $\vv$ is first obtained for each category, by averaging text features of the category name in different language prompts. The image is predicted as the category yielding the highest similarity $\uv^{\top}\vv$. 



\begin{itemize}[leftmargin=2.5mm]
\vspace{1mm}

\item \textit{Random initialized Adaptation.} In the original CLIP paper~\cite{radford2021learning}, to enable model adaptation, a linear classifier with parameters $\Wmat \in \R^{P \times K}$ (similarly, we absorb the bias $\bv$ in $\Wmat$ for simplicity) is added on the projected features, where $\Wmat$ is randomly initialized, shown in Figure~\ref{fig:adaptation} (c) This method often provides good linear probing results, but much worse fine-tuning performance, a surprisingly counter-intuitive observation we have found in our experiments.

\item \textit{Language-initialized Adaptation.} 
We argue that the above issue is caused by the fact that the full capacity of language-augmented visual models is not leveraged. The power of pre-trained language encoder and text inputs must play a vital role in model adaptation. Hence, we propose two language-initialized adaption methods, each of which is ensured as a fair comparison variant for language-augmented and language-free models, respectively. 
$(i)$ {\it Separate-Head.} For the linear head $\Wmat \in \R^{P \times K}$ added on the projection space, we initialize $\Wmat$ with $\Vmat$ (bias terms are initialized as zeros), shown in Figure~\ref{fig:adaptation} (d). In this way, the visual and text heads are separated. 
$(ii)$ {\it Merge-Head.}
To fairly compare with the language-free model adaptation, the linear head should directly be added on the backbone (before the projection layer) to ensure that the same number of trainable parameters are updated. Therefore, we propose to initialize  $\Wmat \in \R^{D \times K}$ in this case with the multiplication result of two linear matrices  $\Wmat_v\Vmat$, shown in Figure~\ref{fig:adaptation} (e).  

\end{itemize}

\paragraph{Discussion.} We highly recommend the proposed language-initialized methods as the standard for the community to adapt the pre-trained language-augmented visual models in their downstream tasks for two reasons: 
$(i)$ This simple method yields surprisingly superior empirical performance, as comprehensively demonstrated in our experiments. It significantly improves the default random initialization method for both linear probing and full model fine-tuning, especially in the few-shot settings.
$(ii)$ It provides an effective mechanism to leverage the external knowledge that is collected for a downstream task in our benchmark. As the knowledge can be concatenated with the original language prompt, then encoded into contextualized text features. In contrast, random initialization would ignore this knowledge source.  We hope the proposed language-initialized method can serve as a strong baseline to encourage the community to further build more efficient adaptation methods. 

In OD, GLIP is a language-augmented detector, whose overall architecture can be simply considered as adding a cross-modal module over the CLIP-like dual-encoder. In GLIP, its linear probing has been implemented via updating $\Wmat_v$ and $\Wmat_t$ in~\cite{li2021grounded}. A prompt-tuning strategy was proposed, by initializing the language input of the cross-modal module as $\Vmat$, and only updating $\Vmat$ in adaptation. This is similar to our language-init strategy. From this perspective, the boundary of linear probing and prompt tuning becomes blurred, with the major difference in if there exist a cross-modal module.

\vspace{-2mm}
\section{Baseline Results}
\vspace{-4mm}
%
In this section, we present the major experimental results with our benchmark to address two research questions. 
\textbf{\texttt{Q1}}: The importance of language in visual model transfer in adaptation stage.
\textbf{\texttt{Q2}}: We identify three playgrounds that our benchmark can help to cultivate research, including sample-efficiency, parameter-efficiency and external knowledge for visual transfer. We also present novel empirical findings as they appear in the specific setting.  
%
\paragraph{Experiment settings}
To make a fair comparison between different methods, we conduct experiments with $\texttt{FP32}$ precision. Our preliminary experiments show that on average $\texttt{FP16}$ and $\texttt{FP32}$ yields similar zero-shot performance, while $\texttt{FP32}$ models outperform  $\texttt{FP16}$ ones on 16 out of 20 datasets. 
% Our main results on IC and OD are summarized in Table~\ref{tab:perf_ic_overall} and Table~\ref{tab:perf_od_overall}, respectively.


 % \subsection{Image Classification}


\begin{table*}[t!]
    \centering
    \footnotesize
    % \setlength{\tabcolsep}{2.8pt}
    \scalebox{0.9}{
    \begin{tabular}{@{}p{2.7cm}@{} l| l |  cll}
    \toprule
       \multicolumn{2}{c|}{ \multirow{2}{*}{Settings} } & \multirow{2}{*}{Init Method}   &  \multicolumn{2}{c}{ 20 IC datasets }  \\
       \cmidrule{4-6} 
       Checkpoint  & Adaptation & &   Zero-shot &  Few-shot (5, 20, 50) & Full  \\
         \midrule
        \multicolumn{5}{l}{\em {\bf Industry Track} (No pre-train data scale limit)} \\
        \multirow{5}{4.2cm}{CLIP \\ (ViT-B32)}
         &  Linear Probing & Random    &  \multirow{5}{0.8cm}{56.64}  &   58.09 {\tiny $\pm$ 2.80}, 69.97 {\tiny $\pm$ 1.30}, 74.09 {\tiny $\pm$ 0.69} & 78.38 \\      
         &  Linear Probing & Language-S  &   & 65.35 {\tiny $\pm$ 1.24}, 71.69 {\tiny $\pm$ 0.93}, 74.89 {\tiny $\pm$ 0.79} & 78.40 \\
         &  Linear Probing & Language-M  &   &65.88 {\tiny $\pm$ 0.79}, 72.05 {\tiny $\pm$ 0.85}, 75.08 {\tiny $\pm$ 0.73} & 78.96 \\
         & Fine-tuning & Random        &    & 29.75 {\tiny $\pm$ 6.64}, 46.76 {\tiny $\pm$ 11.9}, 61.70 {\tiny $\pm$ 9.97} & 77.77 \\    
         & Fine-tuning & Language-S      &   & 63.29 {\tiny $\pm$ 3.18}, 72.19 {\tiny $\pm$ 1.31}, 75.70 {\tiny $\pm$ 1.14} & 79.97 \\  
         \midrule
        \multirow{2}{4.2cm}{Supervised \\(ViT-B32)}         
         &  Linear Probing & Random    &  \multirow{2}{0.8cm}{ -}  & 56.00 {\tiny $\pm$ 2.67}, 67.23 {\tiny $\pm$ 1.66}, 71.35 {\tiny $\pm$ 1.17} & 75.29 \\
         &  Fine-tuning & Random  &   & 58.55 {\tiny $\pm$ 2.58}, 71.27  {\tiny $\pm$ 1.25}, 75.36 {\tiny $\pm$ 1.42} & 80.39 \\
         \midrule
         \multicolumn{5}{l}{\em {\bf Academic Track} (Pre-trained on large established public datasets)} \\
        \multirow{2}{4.2cm}{UniCL \\(Swin-Tiny)}         
         &  Linear Probing & Language-S    &  \multirow{2}{0.8cm}{27.15}  & 54.31 {\tiny $\pm$ 4.15}, 66.42 {\tiny $\pm$ 2.08}, 70.49 {\tiny $\pm$ 1.01} & 74.75 \\      
         &  Fine-tuning & Language-S  &   & 44.75 {\tiny $\pm$ 5.42}, 56.53 {\tiny $\pm$ 5.37}, 67.90 {\tiny $\pm$ 5.31} & 78.48 \\
         \midrule
        \multirow{2}{4.2cm}{Knowledge UniCL \\(Swin-Tiny)}         
         &  Linear Probing & Language-S    &  \multirow{2}{0.8cm}{33.44}  & 55.06 {\tiny $\pm$ 2.36}, 66.26 {\tiny $\pm$ 1.56}, 70.16 {\tiny $\pm$ 1.09} & 74.47 \\      
         &  Fine-tuning & Language-S  &   & 48.41 {\tiny $\pm$ 2.84}, 58.06 {\tiny $\pm$ 4.30}, 71.66 {\tiny $\pm$ 2.02} & 78.05 \\         
        \bottomrule
    \end{tabular}
    }
    \vspace{-0mm}
    \caption{Averaged results on 20 IC datasets. For model adaptation with the language-augmented initialization methods, Language-S and Language-M indicates the separate-head initialization in Figure~\ref{fig:adaptation} (d) and merge-head initialization in Figure~\ref{fig:adaptation} (e), respectively.}
    \label{tab:perf_ic_overall}
      \vspace{-3mm}
\end{table*}
%
\begin{table*}[t!]
    \centering
    \footnotesize
    % \setlength{\tabcolsep}{2.8pt}
    \scalebox{0.9}{
    \begin{tabular}{@{}p{2.0cm}@{} l|  cll}
    \toprule
       \multicolumn{2}{c|}{ \multirow{2}{*}{Settings} }   &  \multicolumn{3}{c}{ 35 OD datasets }  \\
       \cmidrule{3-5} 
       Checkpoint  & Adaptation &    Zero-shot &  Few-shot (1, 3, 5, 10) & Full  \\
         \midrule
         % \multicolumn{5}{l}{\em {\bf Academic Track} (Pre-trained on large established public datasets)} \\
        \multirow{3}{4.2cm}{GLIP \\(Swin-Tiny)}    
         &  Prompt   &   \multirow{3}{0.8cm}{ 19.7}  
         &  29.7{\tiny $\pm$ 0.4}, 36.5{\tiny $\pm$ 0.6}, 39.0{\tiny $\pm$ 1.1}, 41.8{\tiny $\pm$ 1.2} &  54.4 \\    
         &  Linear Probing  &    & 22.2{\tiny $\pm$ 0.1}, 24.4{\tiny $\pm$ 0.2}, 25.1{\tiny $\pm$ 0.2}, 25.6{\tiny $\pm$ 0.6} &  35.2  \\      
         &  Fine-tuning    &   & 32.2{\tiny $\pm$ 0.7}, 39.2{\tiny $\pm$ 0.3}, 42.5{\tiny $\pm$ 0.9}, 49.1{\tiny $\pm$ 0.6}    & 63.2 \\
         \midrule
        \multirow{2}{4.2cm}{DyHead \\(Swin-Tiny)}         
         &  Linear Probing      &  \multirow{2}{0.8cm}{-}  
         & 15.2{\tiny $\pm$ 0.6}, 19.2{\tiny $\pm$ 0.9}, 19.8{\tiny $\pm$ 1.0}, 20.6{\tiny $\pm$ 1.1} &  31.4 \\      
         &  Fine-tuning    &   
         & 25.6{\tiny $\pm$ 0.4}, 37.1{\tiny $\pm$ 0.5},  40.1{\tiny $\pm$ 1.5}, 44.6{\tiny $\pm$ 0.7}    & 63.9 \\ 
        \bottomrule
    \end{tabular}
    }
    \vspace{-0mm}
    \caption{Averaged results on 35 OD datasets.}
    \label{tab:perf_od_overall}
      \vspace{-3mm}
\end{table*}

\subsection{The Role of Language for Vision}
\vspace{-2mm}
\paragraph{Effectiveness of Language-initialized Adaptation Methods.}
%
In Table~\ref{tab:perf_ic_overall}, we benchmark and compare the effectiveness of the proposed language-initialization methods with the checkpoint CLIP ViT-B32. 
The Merge-Head scheme is consistently better than Separate-Head scheme in all settings (though the gain is minor). This is because the latter often have more parameters than the former, as $P=512 < D=768$. 
To ensure fair comparisons with the random initialization of linear head in CLIP~\cite{radford2021learning} (\# trainable parameters is the same), we consider the Separate-Head language-initialization scheme as default, unless the Merge-Head scheme is specified. 

\begin{wrapfigure}{r}{0.48\textwidth}
  \begin{center}
    \includegraphics[width=0.48\textwidth]{figs/language_init_ic.pdf}
  \end{center}
    \vspace{-0mm}
    \caption{Comparison between random- and language- initialized adaptation.
    }
    \vspace{-2pt}
    \label{fig:adaptation_compare_language_random}
\end{wrapfigure}

As shown in Fig.~\ref{fig:adaptation_compare_language_random}, under both linear probe (LP) and fine-tuning (FT) settings, language-based initialization significantly outperforms random initialization in all settings.  Notably, we show that even with very few shots (\eg 2-shots), both our LP and FT is able to outperform the zero-shot CLIP.  This is contradictory to the finding in the original CLIP paper~\cite{radford2021learning}, where zero-shot outperforms linear probing in the fewer shot (less than 4) settings. With the proposed language-init method, one can ensure that few-shot performance is always better than zero-shot, as we essentially reduce to zero-shot when zero iteration is updated in our language-init method.
Moreover, we also find that with the random initialization, FT performs significantly worse than LP under few-shot settings. However, with the language-init, FT starts to outperform LP with more than 20 shots.
Both findings demonstrate the proposed language-based initialization is consistently effective, suggesting that it is a useful and important technique, and should be the standard adaptation method for the recent language-augmented visual models like CLIP.
% de facto 

\paragraph{The Competition of Foundation Models: Language-free vs Language-augmented.} 
We argue that the correct adaptation methods for language-augmented visual models should leverage both the pre-trained visual and text encoder. It is not sufficient to solely transfer from the visual encoder (though the model size is comparable with language-free counterpart), the pre-trained language encoder plays an important role in task transfer.
In Table~\ref{tab:perf_ic_overall}, with language-init adaptation methods, we now see that the language-augmented model (CLIP) consistently outperforms language-free model (Supervised ViT) in all settings, especially for the limited data settings. Further, language-augmented models are able to perform zero-shot task transfer, while traditional language-free models cannot. Similar conclusions can be drawn for OD in Table~\ref{tab:perf_od_overall}. Hence, we recommend the use of language-augmented visual models for task-level transfer.



\begin{figure}[htbp]
   \vspace{-2pt}
   \centering
    \scalebox{1.0}{
    \begin{tabular}{cc}
     \hspace{-2pt}
      \includegraphics[width=0.48\linewidth]{figs/sample_efficiency_ic.pdf}
        & 
      \hspace{-3mm}
      \includegraphics[width=0.48\linewidth]{figs/sample_efficiency_od.pdf}
      
      \vspace{-2mm}
       \\
      (a) IC: Sample Efficiency & 
      (b) OD: Sample Efficiency
      \vspace{4mm} \\
     \hspace{-2pt}
     
    \includegraphics[width=0.46\linewidth]{figs/parameter_efficiency_ic.pdf}      
        & 
    \hspace{-3mm}
      \includegraphics[width=0.45\linewidth]{figs/parameter_efficiency_od.pdf}
       \vspace{-2mm}
       \\
      (c) IC: Parameter Efficiency  & 
      (d) OD: Parameter Efficiency
      \end{tabular}
    }
    \vspace{-0mm}
    \caption{Adaptation efficiency considerations. For IC, comparison of adaptation efficiency between CLIP and supervised ViT (Sup-ViT). For OD, comparison of adaptation efficiency between GLIP and DyHead.}
    \vspace{-0mm}
    \label{fig:adaptation_efficiency}
\end{figure}



\subsection{Playground I: Sample Efficiency}
%
We explore the sample efficiency in Fig.~\ref{fig:adaptation_efficiency} (a) for IC.
First, we find that CLIP-based adaptation consistently outperforms supervised ViT (Sup-ViT) models, and yields a significant 13\% gain in 5-shot settings. Even without any training samples (zero-shot), CLIP outperforms the 5-shot Sup-ViT by 5\% gain.
This suggests that CLIP models allow a better sample efficiency than supervised ViT models.
With more training samples, the performance gap between the two checkpoints becomes smaller, \eg around 1\% with the full data.
%
Furthermore, we find that fine-tuning CLIP yields better performance than linear probing in >20-shot settings, while being worse in the 5-shot setting.  
This is a bit surprising, as it is contradictory to the common convention that fine-tuning is always better than linear probing. We hypothesize this is because fine-tuning tends to over-fit in the scenarios with a large number of trainable parameters and a small number of training samples.
%
Overall, it suggests that fine-tuning CLIP potentially has a better sample efficiency than linear probing, and a better adaptation strategy on fewer-shot settings can be explored in the future. For supervised ViT, FT is always better than LP, the performance gap becomes larger when more samples are used. In 5-shot settings, the gap is minor, which is similar to observations made for supervised CNNs~\cite{yosinski2014transferable,karayev2013recognizing,karianakis2018reinforced}.


As for the comparison of foundation models, we suggest to report the evaluation results on the entire spectrum of sample-efficiency to fully study the behaviors of a pre-trained model. If compute resource is limited, zero-shot or few-shot evaluation can be used as quick assessment.

We explore the sample efficiency for OD in Fig.~\ref{fig:adaptation_efficiency} (b). The conclusion is similar to IC in that language-augmented visual model (\ie GLIP) is more sample-efficient than language-free visual model (\ie DyHead), when the models are adapted using either LP or FT settings. The performance gap is large in the fewer-shot settings and small in the full-shot settings. The difference is that FT consistently outperforms LP in all settings for OD.

\subsection{Playground II: Parameter Efficiency}
We study the parameter efficiency in Fig.~\ref{fig:adaptation_efficiency} (c) for IC.
For CLIP, we experiment two different settings of linear probing CLIP on whether to merge the last two linear projection layers ($\mathbf{W}_v$ and $\mathbf{V}$ in Fig.~\ref{fig:adaptation}).  Merging these two layers in CLIP allows 1.5$\times$ trainable parameters as keeping them separated. 
%
First, it generally shows the trend that a larger number of trainable parameters leads to a better performance, as demonstrated by three curves/scenarios: full-shot CLIP, full-shot Sup-ViT and 5-shot FT. It verifies that LP and FT provide the lower bound and upper bound, in terms of both \#parameter and performance. Most existing parameter-efficient adaptation methods play a trade-off game.
However, in the scenario of 5-shot CLIP, we do notice a slight drop in performance when we further increase the number of trainable parameters to full-model fine-tuning. It suggests that the scenario of adapting language-augmented visual models for data-limited settings is a much more meaningful playground to explore the line of research in parameter-efficient adaptation methods, as the best performance may potentially require an optimal number of trainable parameters, which is less explored so far.


We study the parameter efficiency in Fig.~\ref{fig:adaptation_efficiency} (d) for OD. The overall trend is similar in that better performance comes with more parameters. It turns out that prompt tuning an language-augmented OD model is an effective parameter-efficient approach. For example, prompting is better than linear probing in GLIP. Further, prompt tuning GLIP outperforms fine-tuning DyHead in the 1-shot setting, where the former has less than 0.1\% parameters of the latter. 


\subsection{Playground III: The Benefit of External Knowledge for Vision}
We investigate the effectiveness of external knowledge in Fig.~\ref{fig:gpt3}, measured by zero-shot task transfer performance. First of all, we find that leveraging external knowledge in language-augmented visual models improves upon the knowledge-free counterparts. For example, UniCL is improved from 27.15 to 29.92\textasciitilde33.93, and GLIP-A is improved from 11.53 to 11.70\textasciitilde13.30. Further, for GPT3 knowledge, a larger number of generated knowledge items often leads to higher performance. When combining GPT3 knowledge with Wiktionary knowledge, we see a further performance boost. The gain is consistent for IC, but not consistent for OD with a varying number of GPT3 knowledge items.

In Table~\ref{tab:perf_ic_overall}, we study the role of knowledge for task transfer in model adaptation. Initializing the linear head using encoded features with knowledge is an effective way to leverage the collected knowledge sources, especially for the fewer-shot settings. We also find that it may be insufficient to only use the explicit database knowledge sources such as Wiktionary to initialize the linear head of knowledge UniCL, which sometimes results in instability and lower performance.  We hypothesize this is because the partial knowledge coverage of Wiktionary leads to a situation that some classes are initialized with knowledge, while some are not. It results in two separate embedding clusters, making it difficult to optimize. To solve this, we propose to initialize with both Wiktionary and GPT3 knowledge (which leads to a notable improvement, \eg 1.4\% absolute averaged performance gain in 50-shot FT).

\begin{table}[t!]
	\centering
    \scalebox{0.98}{
    \begin{tabular}{l | cc | cc}
    \toprule
         \multirow{2}{*}{Model} &
         \multicolumn{2}{c|}{5-shot} & \multicolumn{2}{c}{Full-shot} \\
           & LP & FT & LP & FT
          \\          
        \midrule
        CLIP & 65.35 {\tiny $\pm$ 1.24} & 63.29 {\tiny $\pm$ 3.18} & 78.40 & 79.97 \\
        K-CLIP & 65.83 {\tiny $\pm$ 1.50} & 65.10 {\tiny $\pm$ 2.08} & 78.75 & 80.32 \\
        \midrule
        Gain & +0.48 & +1.81 & +0.35 & +0.35 \\
        \# wins & 15/20 & 16/20 & 16/20 & 15/20 \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-0mm}
    \caption{Benefits of external knowledge source to CLIP}
    \label{table:clip_knowledge_gain}
\end{table}

% \begin{figure}[t!]
% 	\centering
% % 	\begin{tabular}{cc}
% % 	\hspace{-4pt}
% % 	\includegraphics[width=0.48\linewidth]{figs/compare_knowledge_clip_wins.pdf}
% % 	& 
% % 	\hspace{-4pt}
% % 	\includegraphics[width=0.48\linewidth]{figs/compare_knowledge_clip_wins.pdf} \vspace{-4pt}	\\
% % 	(a) Knowledge CLIP vs CLIP &
% % 	(b) Knowledge CLIP vs CLIP
% % 	\end{tabular} \\
% 	\vspace{3pt}
%     %
%     \vspace{4pt}
%     \hspace{2mm}
%     \scalebox{0.98}{
%     \begin{tabular}{l | cc | cc}
%     \toprule
%          \multirow{2}{*}{Model} &
%          \multicolumn{2}{c|}{5-shot} & \multicolumn{2}{c}{Full-shot} \\
%           & LP & FT & LP & FT
%           \\          
%         \midrule
%         CLIP & 65.35 {\tiny $\pm$ 1.24} & 63.29 {\tiny $\pm$ 3.18} & 78.40 & 79.97 \\
%         K-CLIP & 65.83 {\tiny $\pm$ 1.50} & 65.10 {\tiny $\pm$ 2.08} & 78.75 & 80.32 \\
%         \midrule
%         Gain & +0.48 & +1.81 & +0.35 & +0.35 \\
%         \# wins & 15/20 & 16/20 & 16/20 & 15/20 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \vspace{-2pt}
%     \caption{Benefits of external knowledge source to CLIP}
%     \label{fig:clip_knowledge_gain}%\vspace{-1.0em}
% \end{figure}

We also explore the benefits of the external knowledge to models that are initially trained without the external knowledge (\eg CLIP). On CLIP, we compare the effect of adding different combinations of external knowledge (Wiktionary, \# of GPT3 queries).  We find that zero-shot CLIP demonstrates consistent improvement on 6 datasets when the external knowledge is available.
% Similarly, linear probing and finetuning CLIP also consistently demonstrate improvement on a specific set of datasets with the external knowledge.
This suggests that the knowledge can benefit the adaptation of vision-language models (though varying between datasets), even if the base model is trained without the external knowledge.

We argue that the model can \emph{selectively} incorporate different knowledge sources to achieve the best adaptation performance.  One simple strategy is to train the model with different knowledge sources, compare the \emph{validation} accuracy of checkpoints with different knowledge sources, and use the best one for testing.  We find such simple strategy is already effective for linear probing and finetuning CLIP.  As shown in Table.~\ref{table:clip_knowledge_gain}, knowledge-CLIP consistently improves over CLIP both in terms of accuracy and \# of wins. Notably, by selectively incorporating the external knowledge, it shows a significant 1.8 improvement for 5-shot CLIP finetuning.  Note that such gain comes for \emph{free} even when the base CLIP model is \emph{not} pretrained with the external knowledge.  We believe more sophisticated knowledge adaptation strategy can yield even better performance and we leave that to future work.  \lht{do we want to put an upper bound here, or it will create some confusion?}

These experiments show that the external knowledge is a very useful resource for improving the adaptation of vision-language models.


\subsection{Comparison with SSL \lht{TODO: move this section}}



\begin{table*}[t!]
    \centering
    \footnotesize
    % \setlength{\tabcolsep}{2.8pt}
    \scalebox{1.0}{
\begin{tabular}{@{}p{2.7cm}@{} l| ccccc}
    \toprule
       \multicolumn{2}{c|}{ \multirow{2}{*}{Settings} }  &  \multicolumn{5}{c}{ 20 Image Classification Datasets }  \\
       \cmidrule{3-7} 
       Checkpoint  & Adaptation &  Zero-shot &  5-shot & 20-shot & 50-shot & Full-shot  \\
        \midrule
        CLIP$^\star$ & Linear Probing & 59.96 & 68.27 {\tiny $\pm$ 0.97} & 74.76 {\tiny $\pm$ 1.11} & 77.75 {\tiny $\pm$ 0.81} & 81.17 \\
        ViT$^\dagger$ & Linear Probing & - & 57.61 {\tiny $\pm$ 3.62} & 69.93 {\tiny $\pm$ 0.71} & 73.74 {\tiny $\pm$ 0.79} & 77.60 \\ 
        DeiT$^\ddagger$ & Linear Probing & - & 54.06 {\tiny $\pm$ 3.02} & 68.57 {\tiny $\pm$ 3.43} & 75.53 {\tiny $\pm$ 0.72} & 79.56 \\ 
        MAE$^\ddagger$ & Linear Probing & - & 33.37 {\tiny $\pm$ 1.98} & 48.03 {\tiny $\pm$ 2.70} & 58.26 {\tiny $\pm$ 0.84} & 68.70 \\  
        MoCo-v3$^\ddagger$ & Linear Probing & - & 50.17 {\tiny $\pm$ 3.43} & 61.99 {\tiny $\pm$ 2.51} & 69.71 {\tiny $\pm$ 1.03} & 74.92 \\
        \midrule
        CLIP$^\star$ & Fine-tuning & 59.96 & 69.12 {\tiny $\pm$ 1.66} & 74.77 {\tiny $\pm$ 2.34} & 78.21 {\tiny $\pm$ 2.04} & 83.63 \\
        ViT$^\dagger$ & Fine-tuning & - & 57.18 {\tiny $\pm$ 2.02} & 72.45 {\tiny $\pm$ 2.85} & 78.53 {\tiny $\pm$ 0.69} & 82.02 \\ 
        DeiT$^\ddagger$ & Fine-tuning & - & 54.06 {\tiny $\pm$ 3.02} & 68.53 {\tiny $\pm$ 3.47} & 75.57 {\tiny $\pm$ 0.68} & 79.55 \\ 
        MAE$^\ddagger$ & Fine-tuning & - & 36.10 {\tiny $\pm$ 3.25} & 54.13 {\tiny $\pm$ 3.86} & 65.86 {\tiny $\pm$ 2.42} & 74.43 \\ 
        MoCo-v3$^\ddagger$ & Fine-tuning & - & 39.30 {\tiny $\pm$ 3.84} & 58.75 {\tiny $\pm$ 5.55} & 70.33 {\tiny $\pm$ 1.64} & 77.71 \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-0mm}
    \caption{Averaged results on 20 IC datasets with ViT-B16 checkpoints. $^\star$ with the proposed language-augmented initialization. $^\dagger$ pretrain on ImageNet21k, then finetune on ImageNet1k. $^\ddagger$ pretrain on ImageNet1k. \lht{TODO: add zero shot}}
    \label{tab:perf_ic_vitb16}
      \vspace{-3mm}
\end{table*}


\begin{figure}[t!]
	\centering
	\begin{tabular}{cc}
	\hspace{-4pt}
	\includegraphics[width=0.48\linewidth]{figs/gpt3/gpt3_knowledge_aggregation_ic.pdf}
	& 
	\hspace{-4pt}
	\includegraphics[width=0.48\linewidth]{figs/gpt3/gpt3_knowledge_aggregation_od.pdf} \vspace{-4pt}	\\
	(a) Image classification &
	(b) Object detection
	\end{tabular} \\
	\vspace{3pt}
    %
    \vspace{4pt}
    \hspace{2mm}
    \scalebox{0.98}{
    \begin{tabular}{l | l c | ccccc}
    \toprule
          \multirow{2}{*}{Problem} 
          & \multirow{2}{*}{Model}
          & \multirow{2}{*}{Baseline}
          & 
         \multicolumn{5}{c}{External Knowledge Sources in Evaluation} \\
           &  &  & 
         $\texttt{wn\_path}$ &  
         $\texttt{wn\_def}$  &  
         $\texttt{wiki\_def}$  &
         $\texttt{gpt3}$  &
         $\texttt{wiki\_def}$ \& $\texttt{gpt3}$
          \\          
        \midrule
        IC &  UniCL
        & \cellcolor{orange!30}27.15 
        & \cellcolor{emerald!30}30.68
        & \cellcolor{emerald!30}29.92
        & \cellcolor{emerald!30}33.44          
        & \cellcolor{emerald!30}33.73         
        & \cellcolor{emerald!30}33.95 \\ 
        %
        OD &  GLIP-A
        & \cellcolor{orange!30}11.53 
        & \cellcolor{emerald!30}12.43
        & \cellcolor{emerald!30}11.70
        & \cellcolor{emerald!30}13.14          
        & \cellcolor{emerald!30}11.98        
        & \cellcolor{emerald!30}13.30 \\         
        \bottomrule
    \end{tabular}
    }    
    \vspace{-2pt}
    \caption{Zero-shot task transfer with various external knowledge sources in the evaluation stage. In (a) and (b), a varying number of generated GPT-3 knowledge sequences is utilized for inference, and ``Wiki-and-GPT3''  indicates both Wiktionary and GPT3 knowledge are used simultaneously. The bottom table summarizes the prediction result for each knowledge source.}
    \label{fig:gpt3}%\vspace{-1.0em}
\end{figure}


% In-context-learning: context = [ classname 1: definition 1 ; classname 2: definition 2; Query/Classname]



\section{Conclusions}
In this paper, we have presented \shortname{}, a platform to evaluate the recently emerging language-augmented visual models for task-level transfer. It consists of 20 image classification datasets and 35 object detection datasets. All of them are collected from public domains, and are enriched with various external knowledge sources to improve the language modality. We have developed open-source toolkits with an auto hyper-parameter pipeline and novel language-initialized adaptation methods to ensure easy utilization and fair comparisons. Strong baseline results are produced from the toolkit to cultivate research in a variety of topics, \eg more transferable language-augmented visual foundation models, advanced model adaption methods (sample-efficiency and parameter-efficiency), and external knowledge for task-level transfer. The question of how to design general-purpose task-level transferable visual models remains largely unanswered. Given benchmarks and tookits we have developed from the perspective of language-augmented visual models, we believe that \shortname{} can provide fertile soil for addressing this challenge.  


\section*{Acknowledgments}
The authors gratefully acknowledge Pengcheng He for helpful discussions to have a separate track dedicated for users from academia, Baolin Peng and and Zhengyuan Yang for the inspirations of GPT3 to generate knowledge for dialogue and OK-VQA tasks. The benchmark depends on publicly available datasets; we acknowledge all the original authors who made their datasets public. Please follow the original license of each dataset and keep this benchmark for academic purposes.

